A Reproducible Extraction of Training Images from Diffusion Models

Recently, Carlini et al. demonstrated the widely used model Stable Diffusion can regurgitate real training samples, which is troublesome from a copyright perspective. In this work, we provide an efficient extraction attack on par with the recent attack, with several order of magnitudes less network evaluations. In the process, we expose a new phenomena, which we dub template verbatims, wherein a diffusion model will regurgitate a training sample largely in tact. Template verbatims are harder to detect as they require retrieval and masking to correctly label. Furthermore, they are still generated by newer systems, even those which de-duplicate their training set, and we give insight into why they still appear during generation. We extract training images from several state of the art systems, including Stable Diffusion 2.0, Deep Image Floyd, and finally Midjourney v4. We release code to verify our extraction attack, perform the attack, as well as all extracted prompts at \url{https://github.com/ryanwebster90/onestep-extraction}.

==> background.tex <==
% \section{Background}


% \paragraph{Diffusion Models}\label{sec:ddpms}
% %%% TODO: TO INTRODUCTION
% Diffusion models have demonstrated state-of-the-art performance on many conditional image generation benchmarks \cite{dhariwal2021diffusion,karras2022elucidating}. Diffusion models are conceptually simple probabilistic models which train a denoising auto encoders. During training, noisy samples are constructed from real ones with a prescribed noise schedule as $z_{t} = \alpha_{t} z_{0} + \sigma_{t} \epsilon$. Here, $\sigma_{t},\alpha_{t}$ are noise levels and scaling factors chosen such that the signal is progressively phased out, i.e. $z_{t}$ becomes a sample of a gaussian distribution $N(0,I\sigma_{T})$. Then, the denoising objective is simply the expectation over the time-steps of the forward diffusion process. Let $D(z_{t},c,t)$ be the conditional denoising auto-encoder conditioned on text $c$, then the loss is simply
% \begin{equation}
% \mathbb{E}_{\epsilon \sim N(0,1), z_{0} \sim p_{data}, t \sim T} \lambda_{t} \left\Vert z_{0} - D(\alpha_{t} z_{0} + \sigma_{t} \epsilon,c, t)) \right\Vert _{2}^{2}
% \end{equation}

% As is noted in \cite{karras2022elucidating}, the diffusion process can be written as an ODE and synthesized images correspond to solutions starting from noise $\sigma_{T}\epsilon$. We found that the Heun sampler, implemented in \cite{kdiffusiongh}, is particularly efficient at synthesis with few iterations compared to other recent sampling techniques \cite{liu2022pseudo,song2022denoising}. We use the Heun sampler throughout this document unless otherwise stated. 

% \paragraph{Data Extraction attacks}
% %

